Efficient Loss-Based Decoding on Graphs For Extreme Classification

In extreme classification problems, learning algorithms are required to map instances to labels from an extremely large label set. We build on a recent extreme classification framework with logarithmic time and space, and on a general approach for error correcting output coding (ECOC) with loss-based decoding, and introduce a flexible and efficient approach accompanied by theoretical bounds. Our framework employs output codes induced by graphs, for which we show how to perform efficient loss-based decoding to potentially improve accuracy. In addition, our framework offers a tradeoff between accuracy, model size and prediction time. We show how to find the sweet spot of this tradeoff using only the training data. Our experimental study demonstrates the validity of our assumptions and claims, and shows that our method is competitive with state-of-the-art algorithms.

==> terms.tex <==
\iffalse

M - coding matrix
L - loss
\ell - coding matrix width (number of predictors/edges)


\epsilon - Average binary loss (as in Allwein) of the hypotheses f_s on the given training set with respect to coding matrix M and loss L
$\eta=\min(\frac{1}{K\ell}\sum_{k,s}^{\frac{M_ks + 1}{2}}, 1-\frac{1}{K\ell}\sum_{k,s}^{\frac{M_ks + 1}{2}})$ - Average subproblem balance % TODO : Define in the paper and explain it behaves like 1/b^2
\rho - Minimum distance
\ell\epsilon = total binary loss
M
OVR - One-vs-rest
AVA - All-vs-All
b - slice width
K - number of classes
d - dimensionality

dichotomizers are out! Use: ** binary learners*

ECOC - Error Correcting Output Codes (define in paper)
vs (not Versus)

Edward complete:
Slice function (For the first part)?


\fi 
